On the Nature of Self-Consistency in Density Functional Theory

A thesis providing a pedagogical introduction to the problem of achieving self-consistency in density functional theory. Contained is an introduction to the framework of Kohn-Sham density functional theory, leading then to the considerations required to solve the equations of Kohn-Sham density functional theory. Specifically, a focus is placed on where current self-consistent field methodology is inefficient and/or fails to converge to a solution. As such, this review spans sub-disciplines such as numerical analysis of linear and non-linear systems, linear response theory, and general electronic structure theory. Toward the end of the thesis, certain contemporary methods for achieving self-consistency from literature are outlined, and a novel, computationally efficient preconditioning strategy is proposed. This work is implemented in the CASTEP software.

==> Chapters/word_count.tex <==
\chapter{Theory} % Main chapter title

\label{sec_2} % For referencing the chapter elsewhere, use \ref{Chapter1} 

\lhead{2. \emph{Theory}} % This is for the header on each page - perhaps a shortened title

%----------------------------------------------------------------------------------------

The problem of achieving self-consistency in KS DFT is a multifaceted one, which spans multiple subdisciplines, such as numerical analysis of linear and non-linear systems, linear response theory, and electronic structure theory (not just limited to KS systems). This chapter will, in some hopefully coherent order, detail why these are all necessary ingredients in solving KS DFT. To do this, one must start with a statement of the overarching problem, which is calculating the electronic structure of a system using quantum theory. The necessity of a framework like KS DFT will then become apparent, and following this, the background of (KS) DFT will be reviewed. This review will end by isolating the specific subsection of KS DFT which the following work pertains to -- self-consistency and density mixing. Here, a clear and detailed statement of the problem to be solved will be provided. Finally, a discussion of the numerical methods employed within DFT software to achieve sef-consistency, and how one can precondition these methods, will follow. So, to begin, what is the electronic structure problem, and why is it difficult?

\section{The Electronic Structure Problem}

The principles of quantum mechanics, developed over the course of approximately two decades in the early twentieth century by some of history's greatest physicists, provides the physical theory underpinning the behaviour of fundamental particles. This includes systems containing the particles that make up everyday matter - protons, neutrons, and electrons. Phenomena arising from the collective behaviour of these three constituents is dubbed condensed matter physics, and this emergent behaviour makes up much of the rich and varied natural world around us. Within quantum mechanics, the complete description of a condensed matter system consisting of protons, neutrons and electrons is given by the quantum state $|\Psi\rangle$, obeying the dynamical equation of motion,
\begin{equation}
\hat{H} |\Psi\rangle = -i \partial_t |\Psi\rangle,
\end{equation} 
which applies universally, for an appropriately constructed Hamiltonian operator\footnote{This equation in fact \textit{does} apply relativistically, but the form of the Hamiltonian operator necessarily changes in accordance with relativity (or, one moves to second quantisation representation of quantum mechanics, leading to the Dirac equation for spin-$\frac{1}{2}$ Fermions).}. Without specifying a basis in which to represent the operators, the total energy operator takes a similar form to that of the total energy variable in classical mechanics,
\begin{equation}
\hat{H} = \frac{1}{2m}\hat{p}^2 + v(\hat{x}).\label{schro}
\end{equation}
The most common basis in which to express Eq$.$ (\ref{schro}) (analytically) is using eigenstates of the position operator, leading to a total energy operator of the following form,
\begin{align}
\hat{H} = -\frac{1}{2m}\nabla^2 + v(\textbf{r}),\label{posbasisH}
\end{align}
now operating on a \textit{wavefunction} $\psi(\textbf{r})$ (the position basis expansion of the quantum state, $|\Psi\rangle$). Given the representation in Eq$.$ (\ref{posbasisH}), one can now begin to construct a Hamiltonian operator which describes a many-body interacting system of charged nuclei and electrons. The potential function will simply describe the Coulomb interactions between all constituents of the system. The Coulomb interaction decays proportional to inverse of distance, therefore a system of interacting nuclei (Greek indices) and electrons (Latin indices) with masses, charges and positions $\{ M_{\mu}, Z_{\mu}, \textbf{R}_{\mu} \}$ and $\{ m_e, e, \textbf{r}_i \}$ respectively is described by the Hamiltonian\footnote{Now, and hereafter unless otherwise stated, using atomic units $m_e = e = \hbar = 4\pi \epsilon_0 = 1$.},
\begin{align}
\hat{H} = -\frac{1}{2} \sum_i \nabla_i^2 - \sum_{\mu} \frac{1}{2M_{\mu}}  \nabla_{\mu}^2 - \sum_{i,\mu} \frac{Z_{\mu}}{|\textbf{r}_i - \textbf{R}_{\mu}|} + \sum_{\mu \neq \nu} \frac{Z_{\mu}Z_{\nu}}{|\textbf{R}_{\nu} - \textbf{R}_{\mu}|} +  \sum_{i \neq j} \frac{1}{|\textbf{r}_i - \textbf{r}_j|}.\label{cmtham}
\end{align}
This expression includes (from left to right): the kinetic energies of the electrons and nuclei (separable additive operators, but crucially are required to operate on the full many-body wavefunction to produce the correct kinetic energy), the electron-nuclear, nuclear-nuclear, and the electron-electron Coulomb interactions.

 The first big simplication in finding a solution to the Schr\"odinger equation is to notice that time can be integrated out, meaning the solution is seperable in the following way,
\begin{gather}
\Psi(\{\textbf{r}_i \}, \{ \textbf{R}_{\mu} \}; t) = \tilde{\Psi}(\{\textbf{r}_i \}, \{ \textbf{R}_{\mu} \}) \Theta(t),\\
 \Theta(t) = e^{-iEt}.
\end{gather}  
This allows time to be included explicitly, and one can focus on finding a \textit{stationary state} solution to the time-independent Schr\"odinger equation,
\begin{align}
\hat{H} |\Psi\rangle = E |\Psi\rangle.
\end{align}
Importantly, provided the operator does not vary in time (which the Hamiltonian above does not) the expectation values of a quantum state (corresponding to the observables that we are interested in calculating) do not vary in time. One is left now with a quantum state, $|\Psi\rangle$, describing a composite system as an eigenstate of the Hamiltonian operator, living in a Hilbert space, $\mathcal{H}$, whose dimension is multiplicative with respect to the number of constituents. This is an important fact, and a quick example can show why the interacting (non-seperable) nature of the system (via the Columb interaction) vastly increases the complexity of the problem. Imagine two, single particle states
\begin{align}
|\phi\rangle, |\psi\rangle \in \mathcal{H}
\end{align}
representing identical particles. Each can be expressed in a infinite basis $\{ |n\rangle \text{ } | \text{ }  n \in [1,\infty] \} $ that spans $\mathcal{H}$. Computationally, one tends to truncate the basis in such a way that (atleast with planewaves) it asymtotically approaches the true Hilbert space,  $\{ |n\rangle \text{ } | \text{ }  n \in [1,b] \}$. Here, $b$ is the total number of basis functions used in the finite representation, and thus parameterises the accuracy of the representation. In a composite interacting system of two identical particles,
\begin{align}
|\Psi\rangle \in \mathcal{H}^{\text{composite}} = \mathcal{H} \otimes \mathcal{H},
\end{align}
the dimension of the truncated composite Hilbert space will be $b^2$. Hence, if a computist finds $b=100$ basis functions provides a reasonable accuracy for resolving the individual single particle states, the solution of their composite system to the same accuracy will have an upper bound requirement $10000$ basis functions. In reality, indistinguishability (i.e$.$ the same basis is used for each constituent) and the exclusion principle mean the complexity increases combinatorically in number of constituants as $^bC_N$. If the above $\{ N=1, b=100 \}$ calculation took, for example, 100 seconds, one might expect a $\{ N=20, b = \Perms{100}{20} \}$ calculation would take something of the order of $10^{22}$ seconds, which is a number perhaps best expressed in units of universe ages (see Fig$.$ \ref{fig:scaling}). 

\begin{figure*}[htbp]
\centering
\includegraphics[width=4in]{scaling.pdf}
\caption{Scaling of the many-body problem: the y-axis represents the combinatorical scaling $t \sim \mathcal{O}(^bC_N)$ with a prefactor for the one electron case of about 60 seconds.}
\label{fig:scaling}
\end{figure*}


Clearly, one needs to find a way to suppress this exponential increase in complexity. The source of this complexity is the interaction terms in the Hamiltonian, which cannot be seperated in an addative fashion with respect to the constituent variables. If they could, the exact solution would take the form of a product state,
\begin{align}
\Psi(\{ \textbf{r}_i \}) = \prod\limits_{i=1}^N \phi_i(\textbf{r}_i);
\end{align}
where each $\phi_i(\textbf{r}_i)$  solves its own seperate Hamiltonian $\hat{h}_i$, requiring a basis resolution $b$. The total composite solution to a given single particle accuracy now only requires $Nb$ basis functions -- the effective dimension of the Hilbert space has become addative with respect to particle number. This defines a system of so-called `non-interacting' particles, which is a core concept behind DFT, and many other electronic structure methods.

The first simplying approximation usually made to Eq$.$ (\ref{cmtham}) in an attempt to reduce the complexity (without much loss of accuracy) is called the \textit{Born-Oppenheimer} approximation, which is responsible for the name of the subdisplcine electronic structure. This approximation functions by noticing that $\frac{1}{M_{\mu}}$ in the nuclear kinetic energy is, in a relative sense, small. This means the kinetic energy contribution of the nuclei to the many-body wavefunction is small if one focuses only on electronic behaviour, and can therefore reasonabley be ignored (this argument is formalised using a power series in the parameter $\frac{1}{M_{\mu}}$ -- see Ref$.$ \citep{martin}, which also defines more preciecly the domain of applicibiltiy of the approximation). If the nuclei are treated as effectively static (with respect to the `equilibration' of electrons), the electron-nuclear interaction term can be replaced by an electron moving in a background potential parameterised by the atomic coordinates. Thus, the electronic state and the nuclear state have become decoupled as their contributions to the Hamtiltonian under this apporixmation are entirely addative with respect to each other. The full wavefunction now takes the form,
\begin{align}
\Psi(\{ \textbf{r}_i \},\{ \textbf{R}_{\mu} \}) = \Psi^{\text{elec}}(\{ \textbf{r}_i \}) \Psi^{\text{nuc}}(\{ \textbf{R}_{\mu} \}),
\end{align}
where the electronic wavefunction now solves its own (electronic) Hamiltonian parameterised by the set of nuclear coordinates $\{ \textbf{R}_{\mu} \}$,
\begin{align}
\hat{H}^{\text{elec}} = -\frac{1}{2} \sum_i \nabla_i^2 +  \sum_{i \neq j} \frac{1}{|\textbf{r}_i - \textbf{r}_j|} + \sum_i v_{\text{ext}}(\textbf{r}_i),\label{elecham}
\end{align}
$v_{\text{ext}}$ being the parameterised term -- the external potential. Solving the Schr\"odinger equation using this Hamiltonian defines what it means to determine the electronic structure of a system. A `system' is therefore entirely specified by a given external potential and electron number. As it stands, one interaction term remains, and dealing with this interaction term has been the source of much work within the field of many-body physics. Some of the most popular methods to do this utilise the concept of a \textit{mean-field} in which independent (`non-interacting') particles respond. The mean-field potential is constructed such that it attempts to mimic the behaviour of the interaction terms; DFT and Hartree-Fock (HF) theory are mean-field theories. This regime has even seen success as a post-DFT method for treating electron correlation with a technique called dynamical mean-field theory (DMFT) \citep{}. Mean-field theories have historically been most successful in describing ground state structural properties of matter, e.g. cell parameters. For excited state (optical) properties however, many-body pertubation theory has been shown to provide a better treatment of the relevent physics. For example, the GW approximation using Hedin's equations \citep{hedin,review}, and the Bethe-Salpeter equation (BSE) \citep{BSE}). To conclude, there are many methods available that attempt to treat the true interacting nature of a system within a computationally tractable framework, each finding success in their own domain of applcability \citep{}. However, due to its relative accuracy and transferrability for the computational cost required to solve it, DFT has emerged as the most widely used method in electronic structure theory. It also provides the starting point for many of the post-DFT perturbative methods quoted, such as DFT+GW \citep{}, DFT+GW+BSE \citep{}.

% A key success of mean-field theory, particularly DFT, is in predicting the structural characteristics of matter; properties like cell parameters can be predicted to within 1$\%$ of experiment \citep{}

%Here, first principles (also, \textit{ab initio}) means to work with the governing laws and equations to the current established level of physical theory -- i.e$.$ without resorting to adjustable parameters fit to empirical data. An \textit{ab initio} method should, in principle, posses a well-defined limit whereby the method converges to the exact solution, e.g$.$ some finite grid spacing tending to zero. In this case, nothing has been chosen by the user to steer the answer.



\section{Density Functional Theory}
\label{DFT}

The core concepts behind DFT are quite seperate from the approximations one makes in order to implement it in practice. In isolation from these approximations, DFT is an exact reformulation of quantum mechanics based on two astonishing theorems. These theorems state that, in principle, no information about a quantum system in the \textit{lowest energy state} of a Hamiltonian is lost by operating on the state such that one retrieves the electron density (a measure of the probability of \textit{any} electron being found at a position \textbf{r}). These theorems are called the Hohenberg-Kohn (HK) theorems \citep{}, and they result in all obseravable properties of a ground state system being determind by the three degrees of freedom in the real-valued electron density $\rho(\textbf{r})$, rather than the $3N$ degrees of freedom in the complex-valued wavefunction. The electron density is defined as such,
\begin{align}
\rho(\textbf{r}) = N \int \prod_{i=2}^N d\textbf{r}_i |\Psi(\textbf{r}, \textbf{r}_2, \dots , \textbf{r}_N) |^2, \label{elecdens}
\end{align}
where here, and throughout the remainder of the thesis, spin will be ignored (although a note on spin in relation to the following work will be given in \S\ref{DFT} -- change).

In detail,

\textbf{HK Theorem I.} \textit{The ground state electron density for a system of interacting electrons is uniquely determined by the external potential.}

\textbf{HK Theorem II.} \textit{As a result of HK Theorem I, a universal (non-system-dependent) functional of the electron density can be defined such that this functional is minimised for the exact ground state electron density.} 

%The HK theorems prove that the total energy of a system (defined by the externel potential) is a \textit{unique} functional of the electron density, and furthermore this functional is variational -- i.e$.$ the electron density which minimises this functional is the ground state electron density.
The proofs for these are formulated under the requirement that the wavefunctions be non-degenerate, and the electron density is so-called $v$-representable. This is a problem, as it is not known if an arbitrary function $f(\textbf{r})$ can be represented as a ground state solution of the Schr\"odinger equation with an external potential $v_{\text{ext}}$. Hence, it may be possible that an (appropriately defined) energy functional can be minimised by a spurious non-$v$-reprsentable electron density. Fortunately, the $v$-representability problem, and the non-degeneracy requirement, were solved by the alternate proof of Levy and Lieb \citep{}. Instead, a functional is defined such that a constrained search over all `$N$-representible' electron densities yeilds a unique minimum (for the ground state density). Unlike $v$-representibility, $N$-representibility is not a problem as it has been proved that an arbitrarty function $f(\textbf{r})$ can be represented by some wavefunction using Eq$.$ (\ref{elecdens}) \citep{} (so spurious minima in the energy functional are avoided). Neither proof will be presented here, but a vast literature discussing both is available \citep{}. 

As it stands, the HK theorems are not useful from the point of view of solving the electronic structure problem, as one still requires the many-body wavefunction in order to construct the electron density. Although, even without a framework in place which renders DFT tractible, a number of observations can be made which indicate its potential. First, if one did define a physically reasonable energy functional, finding the minimum of this functional may require an initial guess of the solution. It is far easier to guess a real-valued function in a 3-dimensional space than a complex-valued function in a $3N$-dimensional space. Moreover, the dimensionality of the phase space one would search in to minimise this functional is far reduced from $3N$ to $3$. The nobel prize winning framework which is able to put these observations to use is a theory proposed by Kohn and Sham in 19XX \citep{}. This theory remains formally exact, but with an unknown `exchange-correlation' term. The amount of energy that this term contributes to the total energy, along with how well simple approximations to it perform, is what makes KS DFT so popular across many applications.

\subsection{Density Functional Theory in the Kohn-Sham Framework}

In order to develop a practical approach to DFT, one needs to define a total energy functional $E[\rho(\textbf{r})]$ such that the minimum of this functional provides the exact (or a good approximation to the exact) interacting ground state energy. Moreover, the computational complexity of this functional (solved via standard variational techniques) should be minimal. The ansatz of Kohn and Sham was formulated by envisioning a non-interacting (and therefore computationally soluble) system of electrons in an effective potential $v_{\text{eff}}$. The question now becomes; does such a  $v_{\text{eff}}$ exist that can uniquely reproduce the exact interacating ground state energy and density? Kohn and Sham showed this to be true, and this mapping defines the famed auxillary KS system of non-interacting electrons.

An outline of the idea behind the KS framework is given as follows: under the assumption that electrons are non-interacting, the many-body wavefunction takes the form of a product state --  $\Psi(\{ \textbf{r}_i \}) = \prod\limits_{i=1}^N \phi_i(\textbf{r}_i)$ (or, a Slater determinant). The resultant $N$ independent wavefunctions $\{ \phi_i \}$ are often referred to as `single particle orbitals', and there exist (foregoing, for now, partial occupancies) precicely $N$ of them due to the exclusion principle allowing only one Fermion in a particlar single particle eigenstate of the Hamiltonian. The KS system is now defined:
\begin{gather}
\Big( -\frac{1}{2} \nabla + v_{\text{eff}}(\textbf{r}) \Big) \phi_i(\textbf{r}) = \epsilon_i \phi_i(\textbf{r}), \label{KS} \\
\rho^{\text{KS}}(\textbf{r}) = \sum_{i \in \text{occupied}} | \phi_i(\textbf{r}) |^2, \\
E^{\text{KS}} = \sum_{i \in \text{occupied}} \epsilon_i  - \text{double counting}, \label{KSe}
\end{gather}
where all quantites are assumed to be ground state, and the first term in Eq$.$ (\ref{KS}) represents the kinetic energy of a non-interacting electron. One now seeks to prove that a  $v_{\text{eff}}$  exists such that,
\begin{gather}
\rho^{\text{KS}}(\textbf{r}) = \rho^{\text{int}}(\textbf{r}) = N \int \prod_{i=2}^N d\textbf{r}_i \text{ } |\Psi(\textbf{r}, \textbf{r}_2, \dots , \textbf{r}_N) |^2, \\
E^{\text{KS}} = E^{\text{int}} = \int  \prod_{i=1}^N d\textbf{r}_i  \text{ }  \Psi^*(\{ \textbf{r}_i \}) \hat{H}^{\text{int}} \Psi(\{ \textbf{r}_i \}).
\end{gather}
To do this, one defines the corresponding energy functional of the system in Eqs$.$ (\ref{KS}) - (\ref{KSe}) as, 
\begin{align}
E^{\text{KS}}[\rho] = T_0[\rho] + \int d\textbf{r} \text{ } v_{\text{eff}}(\textbf{r}) \rho(\textbf{r}),
\end{align}
where $T_0[\rho]$ is the kinetic energy functional of independent electrons. The energy functional of the fully interacting system is,
\begin{gather}
E^{\text{int}}[\rho] = F[\rho] +  \int d\textbf{r} \text{ } v_{\text{ext}}(\textbf{r}) \rho(\textbf{r}), \\
F[\rho] = \langle \Psi_{\text{GS}} | T + v_{ee} |  \Psi_{\text{GS}} \rangle.
\end{gather}
Here, $T$ is the kinetic energy operator on the fully interacting system, and $v_{ee}$ is the Coulomb potential operator. To prove that such a $v_{\text{eff}}$ exists, one can check there exists a density which is the stationary point of both functionals simultenously under some definition of $v_{\text{eff}}$. Note that in determining the stationary points, a constrained variation is needed; the ground state electron density is required to satisfy,
\begin{align}
\int d\textbf{r} \text{ } \rho(\textbf{r}) = N,
\end{align}
so the variation is done using Lagrange multipliers. This leads to,
\begin{gather}
\frac{\delta E^{\text{KS}}[\rho]}{\delta \rho} = \frac{\delta T_0[\rho]}{ \delta \rho} + v_{\text{eff}} + \lambda_{\text{NI}} = 0, \\
\frac{\delta E^{\text{int}}[\rho]}{\delta \rho} = \frac{\delta F[\rho]}{ \delta \rho} + v_{\text{ext}} + \lambda_{\text{I}} = 0,
\end{gather} 
with $\lambda_{\text{I/NI}}$ being the interacting and non-interacting Lagrange multipliers -- these can effectively be dropped here, as the behaviour of the variation can be defined up to constant without loss of generality. Clearly an effective potential can satisfy both of these conditions simolteniously, and this potential is obtained by equating them,
\begin{align}
v_{\text{eff}} = \frac{\delta F[\rho]}{ \delta \rho} -  v_{\text{ext}} -  \frac{\delta T_0[\rho]}{ \delta \rho}.\label{effKS}
\end{align}
The ansatz of Kohn and Sham has been proven: it is possible to define an auxillary non-interacting system which nessacarily (and exactly) reproduces the behaviour of the interacting system\footnote{The problem of $v$-representability has resurfaced, however. It is not possible to say that any electron density resulting from a given external potential in the interacting system will be expressible as a density from some external potential in the non-interacting sytem (and vice versa). This is a problem yet to be solved, but is seemingly mostly benign \citep{birdseyeviewonDFT}.}. One is left with the need to find a computationally tractible approximation to $F[\rho]$ such that this mapping can be utilised. Kohn and Sham did this in analogy with Hartree theory, by replacing the electron-electron interaction by a mean-field `Hartree-potential', and having the kinetic energy operator operate on the non-interacting orbitals, rather than the many-body wavefunction\footnote{Pre-KS, the kinetic energy of the interacting system was often approximated using Thomas-Fermi theory \citep{}.},
\begin{align}
F[\rho] = T_0[\rho] + \frac{1}{2} \int d\textbf{r} d\textbf{r}' \frac{\rho(\textbf{r}) \rho(\textbf{r}')}{|\textbf{r} - \textbf{r}'|} + E_{\text{xc}}[\rho].\label{11111}
\end{align}
The final term here -- the exchange-correlation energy -- is defined as difference between the ground state energy of the Hartree system, and the ground state energy of the exact interacting system. It is named as such because, so far, no explicit reference has been made to the Fermionic nature of the system in relation to the statistics it obeys. That is, upon exchange of two electrons, the wavefunction picks up a negative sign, and is therefore an \textit{antisymmetric} function with respect to its arguments. This has the important consequence of lowering the total energy by tending to seperate electrons with like spin, which is reflected by an additional \textit{exchange energy}, $E_{\text{x}}$. The exchange-correlation energy is simply the sum of the exchange energy and the `correlation energy'. Therefore, correlation (an accurate, computationally tractible treatment of which is the holy grail of electronic structure theory) is defined as difference in energy between Hartree-Fock theory (Hartree theory + an exact treatment of exchange) and the fully interacting theory. Nessacarily this includes a contribution from the fact that the independent particle kinetic energy (obtained from the kinetic energy operator on the indepdent particle states) is not the same as the kinetic operator on the interacting wavefunction. A lot of correlation is wrapped up in this difference, as the Hartree potential would provide an exact description of the Coulomb potential felt by an electron due to its surrounings if not for spurious self-interactions.

Substituting Eq$.$ (\ref{11111}) into Eq$.$ (\ref{effKS}) finally provides a systematic method of appraoching the electronic structure problem within a computationally feasible framework,
\begin{align}
v_{\text{eff}}(\textbf{r}) &= \int d\textbf{r} \text{ } \frac{\rho(\textbf{r})}{|\textbf{r} - \textbf{r}'|} + v_{\text{ext}}(\textbf{r}) + \frac{\delta E_{\text{xc}}[\rho(\textbf{r})]}{\delta \rho(\textbf{r})}, \nonumber \\
 &=  v_{\text{h}} +  v_{\text{ext}} +  v_{\text{xc}},
\end{align}
which is used to construct the KS Hamiltonian, solving the KS equations Eq$.$ (\ref{KS}). The exchange-correlation potential is the only term left requiring approximation, acting to parameterise the degree of ignorance about the correlated nature of electrons. It is worth noting here that there is a certain arbitrary nature with which the exchange-correlation potential was constructed. That is, as a functional \textit{explicitly} defined to satisfy a (non-physical) mathematical mapping between interacting and non-interacting systems\footnote{Non-physical, here, is intended to refer to the fact that a \textit{potential energy} is being constructed in order to fully account for a fundmanetal misrepresentation of the \textit{kinetic energy}.}. As such, one loses a degree of physical meaning within the non-interacting KS system. A direct consequence of this is that all but one of the individual energy eigenvalues of the KS system carry no formal physical meaning (other than their sum being $\sim$ total energy). The eigenvalues have meaning within the framework itself (see, Janek's theorem \citep{}), but the only eigenvalue with true physical meaning (in finite systems) is the highest occupied one, equal to the ionisation energy ( \citep{Exact differential equation for the density and ionization energy of a many-particle system}). A particularly cited example of a problem arising due to the fact that the KS eigenvalues don't carry the meaning one might expect is the so-called band gap problem in DFT. That is, a systematic underestimation of the band gap -- calculated from either the energy difference between the highest occupied and lowest unoccupied orbital energies, or the energy difference between two seperate $N+1$ and $N$ electron ground state systems\footnote{The problem is attributed to a non-analytic `derivative discontinuity' in the exchange-correlation potential with respect to particle number \citep{Density-Functional Theory for Fractional Particle Number:
Derivative Discontinuities of the Energy}.}.

Despite these problems, it is an astonishing fact that, for a lot of materials, the exchange-correlation term accounts for a quite a low
 percentage of the overall ground state energy \citep{}. Consequently, ground state properties of matter, such as stable phases and cell parameters, are predicted by DFT to within 1$\%$ of experiment using only a rudimentary treatment of exchange and correlation. For example, by using the exact exchange-correlation energy functional of the homogenious electron gas -- the \textit{local density approximation} (LDA). Increasing the accuracy of DFT therefore amounts to finding, in some sense, a `better' exchange-correlation functional to model the system at hand. It could be aruged therefore that DFT is not an \textit{ab initio} thoery, because it does not approach the exact solution in some well defined limit (as, for example, a pertubative method would). In this context, the problem of increasing accuracy is explained well in Ref$.$ \citep{}, which conceptualises a `Jacob's ladder' of increasing accuracy, starting from no exchange-correlation to exact exchange-correlation --  passing through the LDA, gradient-based extensions of the LDA, exact (non-local) exchange, and more. 


\subsection{Solving the Kohn-Sham Equations}

The KS equations are restated here as,
\begin{gather}
\Big( -\frac{1}{2} \nabla + v_{\text{ext}}(\textbf{r}) + v_{\text{h}}[\rho^{\text{in}}(\textbf{r}),\textbf{r}] + v_{\text{xc}}[\rho^{\text{in}}(\textbf{r}),\textbf{r}] \Big) \phi_i(\textbf{r}) = \epsilon_i \phi_i(\textbf{r}), \label{kohnsham2}\\
\rho^{\text{out}}(\textbf{r}) = \sum_{i \in \text{occupied}} | \phi_i(\textbf{r}) |^2.\label{elecdens2}
\end{gather}
In constructing the non-interacting KS system of electrons, the fundamental structure of the equations has changed due to the introduction of the Hartree and exchange-correlation potentials. That is, the input to the KS equations now depends explicitly on the output via the electron density. Therefore, in order to even begin solving the above system of equations, one must estimate an initial electron density to use as input, $\rho^{\text{in}}$. Once an initial input density has been specified, the (linear) KS equations can be solved Eq$.$ (\ref{kohnsham2}) -- this involves diagonalisation of the KS Hamiltonian in some basis to find the occupied single particle orbitals. From these single particle orbitals, the \textit{output} electron density is constructed using Eq$.$ (\ref{elecdens2}). The input and output densities are (in general) only equal if one has found the ground state electron density that sloves the KS system. The computational journey one takes starting from an initial guess electron density, arriving at an electron density that solves the KS system is preciecly what it means to achieve \textit{self-consistnecy}. This process is summarised in Fig$.$ (\ref{fig:selfcons}). \\

\begin{figure*}[htbp]
\centering

\begin{tikzpicture}[node distance=2cm]
\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black, fill=red!30]
\tikzstyle{io} = [trapezium, trapezium left angle=70, trapezium right angle=110, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=blue!30]
\tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=orange!30]
\tikzstyle{decision} = [diamond, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=green!30]
\tikzstyle{arrow} = [thick,->,>=stealth]


\node (start) [startstop] {Start};

\node (in1) [io, below of=start] {Guess the initial electron density: $\rho^{\text{in}}(\textbf{r}$)};

\node (pro1) [process, below of=in1, align=center] {Construct the KS Hamiltonian:\\$\hat{H}^{\text{KS}}[\rho^{\text{in}}(\textbf{r})] = -\frac{1}{2} \nabla^2 + v_{\text{eff}}[\rho^{\text{in}}(\textbf{r}),\textbf{r}]$};

\node (pro2) [process, below of=pro1, align=center] {Solve the KS equations to obtain the occupied\\single particle orbitals: $\{ \phi_i \}$};

\node (pro3) [process, below of=pro2] {Calculate the output electron density: $\rho^{\text{out}}(\textbf{r})$};

\node (dec1) [decision, below of=pro3,yshift=-1.2cm] {Is $\rho^{\text{out}}(\textbf{r})=\rho^{\text{in}}(\textbf{r})$?};

\node (pro4) [process, right of=dec1, xshift=4cm] {Construct a new $\rho^{\text{in}}(\textbf{r})$};

\node (stop) [startstop, below of=dec1, yshift=-1.3cm] {Stop: $\{ \phi_i \}$ and $\rho^{\text{*}}(\textbf{r}) = \rho^{\text{out}}(\textbf{r}) = \rho^{\text{in}}(\textbf{r})$ is the solution };


\draw [arrow] (start) -- (in1);
\draw [arrow] (in1) -- (pro1);
\draw [arrow] (pro1) -- (pro2);
\draw [arrow] (pro2) -- (pro3);
\draw [arrow] (pro3) -- (dec1);
\draw [arrow] (dec1) -- node[anchor=east] {Yes} (stop);
\draw [arrow] (dec1) -- node[anchor=south] {No} (pro4);
\draw [arrow] (pro4) |- (pro1);

\end{tikzpicture}




\caption{Flow chart depicting a self-consistent solution to the KS equations.}
\label{fig:selfcons}
\end{figure*}


The above set of equations defines a \textit{non-linear system}. That is, a map that takes an input $\rho^{\text{in}}$ and generates an output $\rho^{\text{out}}$ that is non-linarly related to the input,
\begin{align}
F[\rho^{\text{in}}] = \rho^{\text{out}},
\end{align}
where $F$ hereafter defines the \textit{KS map}. Solving this system amounts to finding a fixed point of the non-linar KS map, $\rho^* =  \rho^{\text{in}} =  \rho^{\text{out}}$, which is typically done using an iterative procedure. This iterative procedure acts to define a sequence, $\{ \rho^{\text{in}}_1, \dots , \rho^{\text{in}}_n \}$, such that $\rho^* =  \rho^{\text{in}}_n$ within some defined tolerence. Ideally, this sequence is generated as robustly and efficiently as possible, which is to say, the sequence will eventually converge, and it does so such that $n$ is minimised. In literature, this is often referred to as the \textit{self-consistent field} (SCF) process, where here the self-consistent field is the density -- a 3-dimensional real scalar field. It should be noted that, self-consistency can be equivilently treated by defining a converging sequence of potentials, or wavefunctions; density has simply been chosen here. The reason for this is that within \textsc{castep}, the default method for achieving self-consistency explicitly functions by updating the electron density. This is not required, and indeed the fallback method within \textsc{castep} updates the single particle orbitals directly such a way that minimisation in error is guaranteed between iterations. This method is called ensemble density functional theory (EDFT), and is extremely robust due to its variational nature, but not nearly as efficient as rivaling techniques. The method itself will not be shown in full detail here, as it is not the focus of the thesis, and in fact the work to follow specifically aims to make EDFT redundant. 



which defines EDFT, a robust fallback method for when the default method does not converge. The default method for achieving self-consistency within \textsc{castep} is called \textit{density mixing} (DM), and combines the input and output densities at each iteration to estimate a new input density. This will be detailed in $\S$\ref{DMsec}. Before defining and exploring DM however, a brief discussion of how DFT is implemented in software will be given. This will serve to motivate the need for and scope of improved DM methods, and also introduce some key concepts of \textit{in silico} DFT that will be utilised in the following work, such as the planewave basis set. 


\subsection{Implementation}

In order to implement a solution to the KS equations, one must first characterise type of system one wishes to solve -- here, that is systems in the \textit{solid state}. The concept of a crystal is therefore introduced as an ordered lattice of atoms, invariant under translation by \textit{primitive lattice vectors}. The set of all integer multiples of the primitive lattice vectors form the infinite, periodic Bravais lattice,
\begin{align}
\Lambda = \{ n_1 \textbf{a}_1 +  n_2 \textbf{a}_2 + n_3 \textbf{a}_3 \text{ } | \text{ } n_i \in \mathbb{Z} \}. \label{brav}
\end{align}
One can therefore construct the full Bravais lattice out of two constituents: a \textit{primitive unit cell}, and a translation of this unit cell by the set of all integer multiples of the primitive lattice vectors (the basis). Here, the elements of the Bravais lattice are atomic positions, and the lattice itself is an approximation to the bulk crystal structure -- a method of reducing an $\sim \mathcal{O}(10^{23})$ size system to that of just a primitive cell and three translation vectors. In order to fully exploit this symmetry, one can invoke \textit{Bloch's theorem}, which vastly simplifies calculations of the wavefunction in periodic systems.

\textbf{Bloch's Theorem}. \textit{If a Hamiltonian is invariant under a translation by \textbf{R}, then the resulting wavefunction will take that of a Bloch form,}
\begin{align}
\psi_{\textbf{k}}(\textbf{r}) = e^{i \textbf{k}.\textbf{r}} u_{\textbf{k}}(\textbf{r}),
\end{align}
\textit{where}  $u_{\textbf{k}}(\textbf{r})$ \textit{is a function with the periodicity of the Hamiltonian,}  $u_{\textbf{k}}(\textbf{r}+\textbf{R}) =  u_{\textbf{k}}(\textbf{r})$.

The quantity $\textbf{k}$ labels the \textit{crystal momentum} -- a conserved quantity under translation by a `reciprocal lattice vector'. Like the Bravais lattice, the reciprocal lattice is defined by the set of all integer translations by three reciprocal lattice vectors on a reciprocal primitive cell, and these two lattices are related via a Fourier transform. Therefore, there exists a range of $\textbf{k}$ on reciprocal lattice in which all information is contained -- a \textit{Brillouin zone}. The first Brillouin zone is a particular type of primitive unit cell on the reciprocal lattice, and is conventionally chosen to be the range of \textbf{k} for which the wavefunction is calculated. 

The wavefunction of the infinity of electrons in the Bravais lattice can now be calculated as the wavefunction within the unit cell, multiplied by a phase labelled by $\textbf{k}$ spanning the first Brillouin zone. This infinity has been transferred from an infinity of electrons, to an infinite set of continuous values of \textbf{k} that need to be sampled within the first Brillouin zone. Fortunately, the energy (and therefore the wavefunctions) are smoothly varying with \textbf{k} \citep{dd}, allowing for a rather course sampling of \textbf{k} within the first Brillouin zone to accurately represent the wavefunction of an infinite crystal. In the language of KS theory, the external potential is now specified by the Bravais lattice; the KS Hamiltonian is therefore invariant under translation (as the kinetic energy operator is), allowing Bloch's theorem to be utilised in practical calculations.


Given Bloch's theorem, the final ingeredient required in order to computationally solve the KS equations is a method of representing the wavefunctions. This is done with a complete set of basis functions, and implementations of KS DFT are typically distingushed between based on the choice of basis. The wavefunction that is being represented is inherantly periodic (with a periodicity defind by the primitive lattice vectors), so a natural basis to consider would be a complete set of functions with the same inherant periodicity as the unit cell. This can be done using \textit{planewaves}, which is the most popular basis set for electronic structure calculations, defined as,
\begin{align}
u(\textbf{r}) = \sum_{\textbf{G}} C_{\textbf{G}} e^{i \textbf{G}.{\textbf{r}}},
\end{align}
where the set of allowed planewaves is defined by the constraint $\textbf{G}.\textbf{R} = 2 \pi n$ -- i.e$.$ the planewaves must have the same periodicity as the unit cell. The full wavefunction expanded in the planewave basis now takes the form,
\begin{align}
\psi_{\textbf{k}}(\textbf{r}) = \sum_{\textbf{G}} C_{\textbf{G+k}} e^{i (\textbf{G+k}).{\textbf{r}}},
\end{align}
for $\textbf{k}$ in the first Brillouin zone. Other than inherant periodiciy and orthogonality, there are a few distinct advantages of a planewave basis. First, the space of vectors \textbf{G} defining the planewaves lies on the reciprical lattice, thus unlocking the fast fourier transform (FFT) as a powerful tool to switch between spaces when convenient. Moreover, there is absolutely no bias in the basis set toward a particular input system. Therefore, the accuracy of the representation converges monotonically with increasing number of planewaves ordered by increasing magnitude of the allowed $\textbf{G}$-vectors\footnote{This fact also makes including time-dependence particularly easy compared to system-tailored basis sets.}. But, in being unbiased, it sows the seeds of its own demise, as the size of the Hamiltonian can become prohibatively large in order to achieve a certain degree of accuracy. In an attempt to remedy this, one can make the observation that \textit{core electrons} -- electrons in orbitals that are extremely localised to the nuclei -- contribute little to the observable properties and behaviour of a system \citep{}. The contribution of core electrons is mostly contained in how they screen the nuclear potential from the \textit{valance electrons}. Therefore, one might think of constructing an effective potential that provides the exact behaviour for valance electrons, without explicitly considering core electrons as degrees of freedom in the system. This is called the \textit{pseudopotential approximation}. It is particularly useful when using a planewave basis set, as orbitals corresponding to core electrons become increasingly oscillatory, owing to the fact that the core states are constrained to be orthogonal to the valance states. Ossicilatory behaviour in the wavefunction requires many planewaves to represent accurately, so the smoothing as a result of the pseudopotential approximation allows one to use a much reduced number of planewaves. There are many popular softwares implementing planewave DFT, some using the pseudopotential approximation, and some `all-electron'\footnote{The software performing all-electron calculations use another method to simplfy the treatment of core electrons; for example the \textit{muffin-tin approximation} \citep{}.}: \textsc{castep} \citep{}, \textsc{vasp} \citep{}, \textsc{abinit} \citep{}, \textsc{quantum espresso} \citep{}, \textsc{wien2k} \citep{},  and many more. 


The ensuing discussion will now restrict specifically to the methodology employed by \textsc{castep}. The KS equations expanded in terms of the planewave basis set take the form,
\begin{align}
\sum_{\textbf{G}'} \Bigg[ \frac{1}{2} |\textbf{k+G}|^2& \delta_{\textbf{GG}'} + v_{\text{ext}}(\textbf{G}-\textbf{G}') \nonumber \\
 & + v_{\text{h}}(\textbf{G}-\textbf{G}') + v_{\text{xc}}(\textbf{G}-\textbf{G}') \Bigg] C_{\textbf{k+G}',i} = \epsilon_{\textbf{k+G},i}  C_{\textbf{k+G},i},
\end{align}
where $i$ here is the so-called \textit{band index}. The naive way to solve these equations would be to construct the full matrix, perform an exact diagonalisation, and use the $N$ lowest energy eigenfunctions and eigenvalues to calculate the electron density and total energy. This is impractical, as exact diagonalsation here is an $\mathcal{O}(N^3_G)$ operation, where $N_G$ is the number of planewaves included in the truncation of the complete planewave basis set. $N_G$ can become as large as $10^6$, therefore the matrix cannot be diagonalised, or even stored in RAM. Instead, an \textit{iterative diagonalisation} is implemented in order to compute only the lowest $N_b << N_G$ energy eigenfunctions and eigenvalues. Without getting into details, this involves an optimisation algorithm (e.g. whatcastepuses) which acts isolate the $N_b$ lowest energy eigenvectors. However, unconstrained, this algorithm would find $N_b$ copies of the lowest energy eigenvector, so a constrained optimisation is needed. That is, the optimisation is performed subject to the constraint that the wavefunctions remain orthogonal. Therefore, each iterative diagonalisation step requires an orthogonalisation step in the subspace of the $N_b$ lowest energy eigenvectors. This is the source of the often quoted `cubic-scaling' nature in DFT implementations. In reality, the scaling of DFT implementations is not that simple (and, in fact, not cubic at all). From Ref$.$ \citep{matt}, the dominant scaling is indeed due to the iterative diagonalsation, but instead scales as $\mathcal{O}(N_k N_G N_b^2)$; where $N_k$ is the number of \textbf{k} points one uses to sample the Brillouin zone\footnote{This scaling is dominant over the scaling of the application of the KS Hamiltonian onto the trial vectors in the optimiser. With a series of clever operations and FFTs, the scaling becomes $\mathcal{O}(N_k N_b N_G \mathrm{log} N_G)$. For example, one would apply the kinetic energy operator in Fourier space, and any local potential operators in real space, as they are both diagonal in their respective spaces and FFTs can move between them.}.

Iterative diagonalisation of the KS Hamiltonian is one of the two major time sinks in a typical DFT calculation. Referring back to the flowchart in Fig$.$ \ref{fig:selfcons}, every time the input density fails to match the output density, the iterative diagonalistion has to be reran for a new input defind by the new electron density one constructs in an attempt to achieve self-consistency. Accelerating DFT therefore amounts to either improving the strategies one uses to solve the KS equations, or reducing the amount that one needs to solve the KS equations in order to find a self-consistent solution. This work focuses on the latter. 




